Towards Variable and Coordinated Holistic Co-Speech Motion Generation

This paper addresses the problem of generating lifelike holistic co-speech motions for 3D avatars, focusing on two key aspects: variability and coordination. Variability allows the avatar to exhibit a wide range of motions even with similar speech content, while coordination ensures a harmonious alignment among facial expressions, hand gestures, and body poses. We aim to achieve both with ProbTalk, a unified probabilistic framework designed to jointly model facial, hand, and body movements in speech. ProbTalk builds on the variational autoencoder (VAE) architecture and incorporates three core designs. First, we introduce product quantization (PQ) to the VAE, which enriches the representation of complex holistic motion. Second, we devise a novel non-autoregressive model that embeds 2D positional encoding into the product-quantized representation, thereby preserving essential structure information of the PQ codes. Last, we employ a secondary stage to refine the preliminary prediction, further sharpening the high-frequency details. Coupling these three designs enables ProbTalk to generate natural and diverse holistic co-speech motions, outperforming several state-of-the-art methods in qualitative and quantitative evaluations, particularly in terms of realism. Our code and model will be released for research purposes at https://feifeifeiliu.github.io/probtalk/.

==> Bibs/strings.tex <==
% from talkshow
@String(PAMI 	=	{{Transactions on Pattern Analysis and Machine Intelligence (TPAMI)}})
@String(IJCV 	=	{{International Journal of Computer Vision (IJCV)}})
@String(CVPR 	=	{{Computer Vision and Pattern Recognition (CVPR)}})
@String(CVPRW 	=	{{Computer Vision and Pattern Recognition Workshops (CVPRw)}})
@String(ICCV 	=	{{International Conference on Computer Vision ({ICCV})}})
@String(ICCVW 	=	{{International Conference on Computer Vision Workshops (ICCVw)}})
@String(ECCV 	=	{{European Conference on Computer Vision (ECCV)}})
@String(ECCVW 	=	{{European Conference on Computer Vision Workshops (ECCVw)}})
@String(ACCV 	=	{{Asian Conference on Computer Vision (ACCV)}})
@String(ACCVw 	=	{{Asian Conference on Computer Vision Workshops (ACCVw)}})
@String(BMVC 	=	{{British Machine Vision Conference (BMVC)}})
@String(TOG 	=	{{Transactions on Graphics (TOG)}})
@String(SCA 	=	{{Symposium on Computer Animation (SCA)}})
@String(TVCG 	=	{{Transactions on Visualization and Computer Graphics (TVCG)}})
@String(ICLR 	=	{{International Conference on Learning Representations (ICLR)}})
@STRING(I3DV 	=	{{International Conference on 3D Vision (3DV)}})
@STRING(CVIU 	=	{{Computer Vision and Image Understanding (CVIU)}})
@STRING(CGF 	=	{{Computer Graphics Forum (CGF)}})
@STRING(RAM 	=	{{Robotics \& Automation Magazine (RAM)}})
@STRING(CAGD	=	{{Computer Aided Geometric Design (CAGD)}})
@STRING(CG 		=	{{Computers \& Graphics (CG)}})
@STRING(SIGG	=	{{International Conference on Computer Graphics and Interactive Techniques (SIGGRAPH)}})
@STRING(ICML	=	{{International Conference on Machine Learning (ICML)}})

@STRING(FG 		=	{{International Conference on Automatic Face \& Gesture Recognition (FG)}})
@STRING(AAAI	=	{{AAAI Conference on Artificial Intelligence}})
@String(NEURIPS	=   {{Conference on Neural Information Processing Systems (NeurIPS)}})
@String(TCSVT	=   {{Transactions on Circuits and Systems for Video Technology (TCSVT)}})

@String(COSN	=   {{Conference on Online Social Networks (COSN)}})
@String(CGIP	=   {{Computer Vision, Graphics, and Image Processing (CGIP)}})atla
@String(MVA	    =   {{Machine Vision and Applications (MVA)}})
@String(SI3D	=   {{Symposium on Interactive 3D Graphics (SI3D)}})
@String(JOV	    =   {{Journal of Vision (JOV)}})
@String(WACV	=   {{Winter Conference on Applications of Computer Vision (WACV)}})
@String(GCPR	=   {{German Conference on Pattern Recognition (GCPR)}})
@STRING(ICRA 		=	{{International Conference on Robotics and Automation (ICRA)}})
@STRING(TMM 		=	{{Transactions on Multimedia (TMM)}})
@STRING(IVA 		=	{{International Conference on Intelligent Virtual Agents (IVA)}})
@STRING(MM 		=	{{International Conference on Multimedia (MM)}})
@STRING(HCI 		=	{{International Conference on Human-Computer Interaction (HCI)}})
@STRING(EMNLP 		=	{{Conference on Empirical Methods in Natural Language Processing (EMNLP)}})
@STRING(IROS 		=	{{International Conference on Intelligent Robots and Systems (IROS)}})
@STRING(ICMI 		=	{{International Conference on Multimodal Interaction (ICMI)}})
@STRING(SC 		=	{{Speech Communication}})

% original siga
@String{AMSTrans = "American Mathematical Society Translations" }
@String{AMSTrans = "Amer. Math. Soc. Transl." }
@String{BullAMS = "Bulletin of the American Mathematical Society" }
@String{BullAMS = "Bull. Amer. Math. Soc." }
@String{ProcAMS = "Proceedings of the American Mathematical Society" }
@String{ProcAMS = "Proc. Amer. Math. Soc." }
@String{TransAMS = "Transactions of the American Mathematical Society" }
@String{TransAMS = "Trans. Amer. Math. Soc." }

%ACM
@String{CACM = "Communications of the {ACM}" }
@String{CACM = "Commun. {ACM}" }
@String{CompServ = "Comput. Surveys" }
@String{JACM = "J. ACM" }
@String{ACMMathSoft = "{ACM} Transactions on Mathematical Software" }
@String{ACMMathSoft = "{ACM} Trans. Math. Software" }
@String{SIGNUM = "{ACM} {SIGNUM} Newsletter" }
@String{SIGNUM = "{ACM} {SIGNUM} Newslett." }

@String{AmerSocio = "American Journal of Sociology" }
@String{AmerStatAssoc = "Journal of the American Statistical Association" }
@String{AmerStatAssoc = "J. Amer. Statist. Assoc." }
@String{ApplMathComp = "Applied Mathematics and Computation" }
@String{ApplMathComp = "Appl. Math. Comput." }
@String{AmerMathMonthly = "American Mathematical Monthly" }
@String{AmerMathMonthly = "Amer. Math. Monthly" }
@String{BIT = "{BIT}" }
@String{BritStatPsych = "British Journal of Mathematical and Statistical
      Psychology" }
@String{BritStatPsych = "Brit. J. Math. Statist. Psych." }
@String{CanMathBull = "Canadian Mathematical Bulletin" }
@String{CanMathBull = "Canad. Math. Bull." }
@String{CompApplMath = "Journal of Computational and Applied Mathematics" }
@String{CompApplMath = "J. Comput. Appl. Math." }
@String{CompPhys = "Journal of Computational Physics" }
@String{CompPhys = "J. Comput. Phys." }
@String{CompStruct = "Computers and Structures" }
@String{CompStruct = "Comput. \& Structures" }
@String{CompJour = "The Computer Journal" }
@String{CompJour = "Comput. J." }
@String{CompSysSci = "Journal of Computer and System Sciences" }
@String{CompSysSci = "J. Comput. System Sci." }
@String{Computing = "Computing" }
@String{ContempMath = "Contemporary Mathematics" }
@String{ContempMath = "Contemp. Math." }
@String{Crelle = "Crelle's Journal" }
@String{GiornaleMath = "Giornale di Mathematiche" }
@String{GiornaleMath = "Giorn. Mat." } % didn't find in AMS MR., ibid.

%IEEE
@String{Computer = "{IEEE} Computer" }
@String{IEEETransComp = "{IEEE} Transactions on Computers" }
@String{IEEETransComp = "{IEEE} Trans. Comput." }
@String{IEEETransAC = "{IEEE} Transactions on Automatic Control" }
@String{IEEETransAC = "{IEEE} Trans. Automat. Control" }
@String{IEEESpec = "{IEEE} Spectrum" } % didn't find in AMS MR
@String{ProcIEEE = "Proceedings of the {IEEE}" }
@String{ProcIEEE = "Proc. {IEEE}" } % didn't find in AMS MR
@String{IEEETransAeroElec = "{IEEE} Transactions on Aerospace and Electronic
 Systems" }
@String{IEEETransAeroElec = "{IEEE} Trans. Aerospace Electron. Systems" }

@String{IMANumerAna = "{IMA} Journal of Numerical Analysis" }
@String{IMANumerAna = "{IMA} J. Numer. Anal." }
@String{InfProcLet = "Information Processing Letters" }
@String{InfProcLet = "Inform. Process. Lett." }
@String{InstMathApp = "Journal of the Institute of Mathematics and
 its Applications" }
@String{InstMathApp = "J. Inst. Math. Appl." }
@String{IntControl = "International Journal of Control" }
@String{IntControl = "Internat. J. Control" }
@String{IntNumerEng = "International Journal for Numerical Methods in
 Engineering" }
@String{IntNumerEng = "Internat. J. Numer. Methods Engrg." }
@String{IntSuper = "International Journal of Supercomputing Applications" }
@String{IntSuper = "Internat. J. Supercomputing Applic." } % didn't find
%% in AMS MR
@String{Kibernetika = "Kibernetika" }
@String{JResNatBurStand = "Journal of Research of the National Bureau
 of Standards" }
@String{JResNatBurStand = "J. Res. Nat. Bur. Standards" }
@String{LinAlgApp = "Linear Algebra and its Applications" }
@String{LinAlgApp = "Linear Algebra Appl." }
@String{MathAnaAppl = "Journal of Mathematical Analysis and Applications" }
@String{MathAnaAppl = "J. Math. Anal. Appl." }
@String{MathAnnalen = "Mathematische Annalen" }
@String{MathAnnalen = "Math. Ann." }
@String{MathPhys = "Journal of Mathematical Physics" }
@String{MathPhys = "J. Math. Phys." }
@String{MathComp = "Mathematics of Computation" }
@String{MathComp = "Math. Comp." }
@String{MathScand = "Mathematica Scandinavica" }
@String{MathScand = "Math. Scand." }
@String{TablesAidsComp = "Mathematical Tables and Other Aids to Computation" }
@String{TablesAidsComp = "Math. Tables Aids Comput." }
@String{NumerMath = "Numerische Mathematik" }
@String{NumerMath = "Numer. Math." }
@String{PacificMath = "Pacific Journal of Mathematics" }
@String{PacificMath = "Pacific J. Math." }
@String{ParDistComp = "Journal of Parallel and Distributed Computing" }
@String{ParDistComp = "J. Parallel and Distrib. Comput." } % didn't find
%% in AMS MR
@String{ParComputing = "Parallel Computing" }
@String{ParComputing = "Parallel Comput." }
@String{PhilMag = "Philosophical Magazine" }
@String{PhilMag = "Philos. Mag." }
@String{ProcNAS = "Proceedings of the National Academy of Sciences
                of the USA" }
@String{ProcNAS = "Proc. Nat. Acad. Sci. U. S. A." }
@String{Psychometrika = "Psychometrika" }
@String{QuartMath = "Quarterly Journal of Mathematics, Oxford, Series (2)" }
@String{QuartMath = "Quart. J. Math. Oxford Ser. (2)" }
@String{QuartApplMath = "Quarterly of Applied Mathematics" }
@String{QuartApplMath = "Quart. Appl. Math." }
@String{RevueInstStat = "Review of the International Statisical Institute" }
@String{RevueInstStat = "Rev. Inst. Internat. Statist." }

%SIAM
@String{JSIAM = "Journal of the Society for Industrial and Applied
 Mathematics" }
@String{JSIAM = "J. Soc. Indust. Appl. Math." }
@String{JSIAMB = "Journal of the Society for Industrial and Applied
 Mathematics, Series B, Numerical Analysis" }
@String{JSIAMB = "J. Soc. Indust. Appl. Math. Ser. B Numer. Anal." }
@String{SIAMAlgMeth = "{SIAM} Journal on Algebraic and Discrete Methods" }
@String{SIAMAlgMeth = "{SIAM} J. Algebraic Discrete Methods" }
@String{SIAMAppMath = "{SIAM} Journal on Applied Mathematics" }
@String{SIAMAppMath = "{SIAM} J. Appl. Math." }
@String{SIAMComp = "{SIAM} Journal on Computing" }
@String{SIAMComp = "{SIAM} J. Comput." }
@String{SIAMMatrix = "{SIAM} Journal on Matrix Analysis and Applications" }
@String{SIAMMatrix = "{SIAM} J. Matrix Anal. Appl." }
@String{SIAMNumAnal = "{SIAM} Journal on Numerical Analysis" }
@String{SIAMNumAnal = "{SIAM} J. Numer. Anal." }
@String{SIAMReview = "{SIAM} Review" }
@String{SIAMReview = "{SIAM} Rev." }
@String{SIAMSciStat = "{SIAM} Journal on Scientific and Statistical
 Computing" }
@String{SIAMSciStat = "{SIAM} J. Sci. Statist. Comput." }

@String{SoftPracExp = "Software Practice and Experience" }
@String{SoftPracExp = "Software Prac. Experience" } % didn't find in AMS MR
@String{StatScience = "Statistical Science" }
@String{StatScience = "Statist. Sci." }
@String{Techno = "Technometrics" }
@String{USSRCompMathPhys = "{USSR} Computational Mathematics and Mathematical
 Physics" }
@String{USSRCompMathPhys = "{U. S. S. R.} Comput. Math. and Math. Phys." }
@String{VLSICompSys = "Journal of {VLSI} and Computer Systems" }
@String{VLSICompSys = "J. {VLSI} Comput. Syst." }
@String{ZAngewMathMech = "Zeitschrift fur Angewandte Mathematik und
 Mechanik" }
@String{ZAngewMathMech = "Z. Angew. Math. Mech." }
@String{ZAngewMathPhys = "Zeitschrift fur Angewandte Mathematik und Physik" }
@String{ZAngewMathPhys = "Z. Angew. Math. Phys." }

% Publishers % ================================================= |

@String{Academic = "Academic Press" }
@String{ACMPress = "{ACM} Press" }
@String{AdamHilger = "Adam Hilger" }
@String{AddisonWesley = "Addison-Wesley" }
@String{AllynBacon = "Allyn and Bacon" }
@String{AMS = "American Mathematical Society" }
@String{Birkhauser = "Birkha{\"u}ser" }
@String{CambridgePress = "Cambridge University Press" }
@String{Chelsea = "Chelsea" }
@String{ClaredonPress = "Claredon Press" }
@String{DoverPub = "Dover Publications" }
@String{Eyolles = "Eyolles" }
@String{HoltRinehartWinston = "Holt, Rinehart and Winston" }
@String{Interscience = "Interscience" }
@String{JohnsHopkinsPress = "The Johns Hopkins University Press" }
@String{JohnWileySons = "John Wiley and Sons" }
@String{Macmillan = "Macmillan" }
@String{MathWorks = "The Math Works Inc." }
@String{McGrawHill = "McGraw-Hill" }
@String{NatBurStd = "National Bureau of Standards" }
@String{NorthHolland = "North-Holland" }
@String{OxfordPress = "Oxford University Press" }  %address Oxford or London?
@String{PergamonPress = "Pergamon Press" }
@String{PlenumPress = "Plenum Press" }
@String{PrenticeHall = "Prentice-Hall" }
@String{SIAMPub = "{SIAM} Publications" }
@String{Springer = "Springer-Verlag" }
@String{TexasPress = "University of Texas Press" }
@String{VanNostrand = "Van Nostrand" }
@String{WHFreeman = "W. H. Freeman and Co." }

==> Sections/RebFig_User.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.95\columnwidth]{Figures/rebuttal/user(1).pdf}
    % \vspace{-0.05in}
    % \vspace{-0.3in}
    % \captionsetup{font=scriptsize}
    % \caption{User study.}
    \vspace{-0.3in}
    \label{fig:user_study}
\end{figure}

==> Tables/Tab_06_ABLA_CONTI.tex <==
\begin{table*}[t]
    \footnotesize
    \centering
    \resizebox{0.4\linewidth}{!}{
    \begin{tabular}{cc|cccccccc}
    \toprule
    Motion Context & Refiner
    & \tabincell{c}{FGD $\downarrow$}
    & \tabincell{c}{BC $\uparrow$}
    & \tabincell{c}{MAJE $\downarrow$}
    & \tabincell{c}{MAD $\downarrow$}
    \\\hline
        &                   & 13.64 & 0.293 & 0.604 & 0.0215 \\
    \checkmark &            & 16.33 & 0.362 & 0.641 & 0.0225 \\
    \checkmark & \checkmark & 12.09 & 0.745 & 0.557 & 0.0239 \\ \hline
    \end{tabular}
    }
    \caption{Ablation context motion frames.}
    \label{tab:ablation}
    
\end{table*}
